Two-loop matching of renormalizable operators: general considerations and applications

Low-energy effective field theories (EFT) encode information about the physics at high energies--i.e., the high-energy theory (HET). To extract this information the EFT and the HET have to be matched to each other. At the one-loop level, general results for the matching of renormalizable operators have already been obtained in the literature. In the present paper, we take a step towards a better understanding of renormalizable operator matching at the two-loop level: Focusing on the diagrammatic method, we discuss in detail the various contributions to two-loop matching conditions and compare different approaches to derive them. Moreover, we discuss which observables are best suited for the derivation of matching conditions. As a concrete application, we calculate the $\mathcal{O}\left(\alpha_t \alpha_s \right)$ and $\mathcal{O} \left(\alpha_t^2 \right)$ matching conditions of the scalar four-point couplings between the Standard Model (SM) and the Two-Higgs-Doublet Model (THDM) as well as the THDM and the Minimal Supersymmetric Standard Model (MSSM). We use the derived formulas to improve the prediction of the SM-like Higgs mass in the MSSM using the THDM as EFT.

==> diag_sec02.tex <==
\begin{figure}[!htb]
  \centering
  \fontsize{12}{12}
  \begin{axopicture}{(400,150)(0,0)}
    \Line[](60,20)(80,40)
    \Line[](140,40)(160,20)
    \Line[](140,100)(160,120)
    \Line[](80,100)(60,120)
    \Line[](80,40)(140,40)
    \Line[](80,40)(80,100)
    \Line[](80,100)(140,100)
    \Line[](140,40)(140,100)
    \Line[](110,40)(110,100)
    \Text(70,70)[]{$m$}
    %
    \Line[](190,20)(210,40)
    \Line[](270,40)(290,20)
    \Line[](270,100)(290,120)
    \Line[](210,100)(190,120)
    \DashLine(210,40)(270,40){3}
    \DashLine(210,40)(210,100){3}
    \DashLine(210,100)(270,100){3}
    \DashLine(270,40)(270,100){3}
    \Line[](240,40)(240,100)
    \Text(200,70)[]{$M$}    
  \end{axopicture}
  \caption{Examples of diagrams contributing to $\Gamma^{(4\phi)}_\text{\HET,light}$ (left) and $\Gamma^{(4\phi)}_\text{\HET,heavy}$ (right).}
  \label{Sec02:example}
\end{figure}

